Structure-Preserving Graph Kernel for Brain Network Classification

This paper presents a novel graph-based kernel learning approach for connectome analysis. Specifically, we demonstrate how to leverage the naturally available structure within the graph representation to encode prior knowledge in the kernel. We first proposed a matrix factorization to directly extract structural features from natural symmetric graph representations of connectome data. We then used them to derive a structure-persevering graph kernel to be fed into the support vector machine. The proposed approach has the advantage of being clinically interpretable. Quantitative evaluations on challenging HIV disease classification (DTI- and fMRI-derived connectome data) and emotion recognition (EEG-derived connectome data) tasks demonstrate the superior performance of our proposed methods against the state-of-the-art. Results showed that relevant EEG-connectome information is primarily encoded in the alpha band during the emotion regulation task.

==> sec_conclusion.tex <==

\section{Conclusion and Future Work}\label{sec:end}

In this paper, we have proposed a multi-view machine (MVM) model and presented a stochastic gradient descent (SGD) learning method with a distributed implementation on Spark. In general, the model is particularly designed for data that is composed of features from multiple views, between which the full-order interactions are effectively explored. In contrast to other models that include only partial feature interactions or factorize different orders of interactions separately, MVMs jointly factorize the full-order feature interactions and thereby benefiting parameter estimation under sparsity and rendering the model with the capacity to avoid overfitting. Moreover, MVMs can be applied to a variety of supervised machine learning tasks, including classification and regression. Empirical studies on real-world web application datasets demonstrate the effectiveness of MVMs on modeling feature interactions in multi-view data, which outperform baseline models for multi-view prediction.

The MVM model can be further investigated in several directions for future work. For example, in addition to SGD, we are interested in implementation of other learning algorithms in a distributed environment to facilitate convergence efficiency, {\em e.g.}, alternating least square (ALS) and Markov Chain Monto Carlo (MCMC) for MVMs. It is also interesting to have our model applied to other multi-view prediction problems. Moreover, defining an evaluation metric for an effective view segmentation would be critical for the subsequent multi-view learning.

\balance
\bibliographystyle{plain}
%\bibliographystyle{abbrv}
%\bibliographystyle{finplain}
\bibliography{reference}

==> table_baseline.tex <==
\begin{table*}
\centering
\caption{Summary of related work. Model complexity refers to both the number of parameters in the model and the time complexity to compute the decision function.}
\label{tab:baseline}
\begin{tabular}{lccc}
\toprule
Method & Model complexity & Feature interactions & Parameter factorization \\
\midrule
Support vector machines (SVMs) \cite{vapnik2000nature} & $O(d)$ & first-order & none \\
Support tensor machines (STMs) \cite{tao2005supervised} & $O(kd)$ & highest-order & factorized ($k=1$ \cite{cao2014tensor}) \\
Factorization machines (FMs) \cite{rendle2010factorization} & $O(kmd)$ & up to full-order & partially and independently factorized \\
Multi-view machines (MVMs) & $O(k(m+d))$ & full-order & fully and jointly factorized \\
\bottomrule
\end{tabular}
\end{table*}

==> table_dataset.tex <==
%\begin{table}[t]
%\centering
%\caption{The statistics and parameters for each dataset. The number in braces indicates the dimensionality of the corresponding view.}
%\label{tab:dataset}
%\begin{tabular}{l|c|c}
%\toprule
%Dataset &{\ml} &{\bing} \\
%\midrule
%views       &users (138,493)            &queries (958,426)      \\
%            &movies (27,278)            &ad URLs (1,935,510)   \\
%            &impl. (27,278)             &impressions (18)       \\
%$n$         &20,000,263                 &28,622,281             \\
%$\eta$      &0.1                        &0.1                    \\
%$\lambda$   &0.01                       &0.01                   \\
%$k$         &20                         &20                     \\
%\bottomrule
%\end{tabular}
%\end{table}

\begin{table*}
\centering
\caption{The statistics and parameters for each dataset. The number in braces indicates the dimensionality of the corresponding view.}
\label{tab:dataset}
\begin{tabular}{lcccccc}
\toprule
Dataset & Views & $n$ & $\eta$ & $\lambda$ & $k$ & \#iterations \\
\midrule
{\ml} & users (138,493), movies (27,278), impl. (27,278) & 20,000,263 & 0.1 & 0.01 & 20 & 200 \\
{\bing} & queries (958,426), ad URLs (1,935,510), impressions (18) & 28,622,281 & 0.1 & 0.01 & 20 & 200 \\
\bottomrule
\end{tabular}
\end{table*}

==> table_example.tex <==
\begin{table}
\centering
\caption{An example showing the discrepancy between feature interactions with different orders. $\#1=user+ad+query$, $\#2=user\times ad+user\times query+ad\times query$, $\#3=user\times ad\times query$.}
\label{tab:example}
\begin{tabular}{ccc|ccc}
\toprule
User & Ad & Query & \#1 & \#2 & \#3 \\
\midrule
1.20 \color{green}{\tiny(+)} & 1.80 \color{green}{\tiny(+)} & 0.50 \color{green}{\tiny(+)}
& 3.50 \color{green}{\tiny(+)} & 3.66 \color{green}{\tiny(+)} & 1.08 \color{green}{\tiny(+)} \\
1.20 \color{green}{\tiny(+)} & 1.80 \color{green}{\tiny(+)} & -0.50 \color{red}{\tiny(-)}
& 2.50 \color{green}{\tiny(+)} & 0.66 \color{green}{\tiny(+)} & -1.08 \color{red}{\tiny(-)} \\
1.20 \color{green}{\tiny(+)} & -1.80 \color{red}{\tiny(-)} & -0.50 \color{red}{\tiny(-)}
& -1.10 \color{red}{\tiny(-)} & -1.86 \color{red}{\tiny(-)} & 1.08 \color{green}{\tiny(+)} \\
\bottomrule
\end{tabular}
\end{table}

==> table_notation.tex <==
\begin{table}
\small
\caption{Symbols.}
\label{tab:notation}
\begin{tabular}{ll}
\toprule
Symbol & Definition and description\\
\midrule
$s$ & each lowercase letter represents a scale\\
$\mathbf{v}$ & each boldface lowercase letter represents a vector\\
$\mathbf{M}$ & each boldface capital letter represents a matrix\\
$\mathcal{T}$ & each calligraphic letter represents a tensor, set or space\\
$[m:n]$ & a set of integers in the range of $m$ to $n$ inclusively. \\
$\left\langle\cdot,\cdot\right\rangle$ & denotes inner product\\
$\circ$ & denotes tensor product or outer product\\
$\odot$ & denotes Hadamard (entrywise) product\\
$\times_k$ & denotes mode-$k$ product\\
$\left|\cdot\right|$ & denotes absolute value\\
$\left\|\cdot\right\|_{F}$ & denotes (Frobenius) norm of vector, matrix or tensor\\
\bottomrule
\end{tabular}
\end{table}


==> table_result.tex <==
\begin{table}
\centering
\caption{Prediction accuracy. {\color{red}{$\downarrow$}} indicates the smaller the value the better the performance; {\color{green}{$\uparrow$}} indicates the larger the value the better the performance.}
\label{tab:exp}
\begin{tabular}{lcc}
\toprule
Dataset &{\ml} (RMSE) \color{red}{$\downarrow$} &{\bing} (AUC) \color{green}{$\uparrow$} \\
\midrule
\mvm        &0.8376      &0.7917            \\
\fm         &0.8681      &0.7872            \\
\bsfm       &0.8447      &0.7729            \\
\threewayfm &0.9060      &0.7201            \\
\partialmvm &0.9807      &0.6947            \\
\tf         &0.8572      &0.6645            \\
\lr         &1.0017      &0.7450            \\
\bottomrule
\end{tabular}
\end{table}
